Progressive Compositionality in Text-to-Image Generative Models

Despite the impressive text-to-image (T2I) synthesis capabilities of diffusion models, they often struggle to understand compositional relationships between objects and attributes, especially in complex settings. Existing solutions have tackled these challenges by optimizing the cross-attention mechanism or learning from the caption pairs with minimal semantic changes. However, can we generate high-quality complex contrastive images that diffusion models can directly discriminate based on visual representations? In this work, we leverage large-language models (LLMs) to compose realistic, complex scenarios and harness Visual-Question Answering (VQA) systems alongside diffusion models to automatically curate a contrastive dataset, ConPair, consisting of 15k pairs of high-quality contrastive images. These pairs feature minimal visual discrepancies and cover a wide range of attribute categories, especially complex and natural scenarios. To learn effectively from these error cases, i.e., hard negative images, we propose EvoGen, a new multi-stage curriculum for contrastive learning of diffusion models. Through extensive experiments across a wide range of compositional scenarios, we showcase the effectiveness of our proposed framework on compositional T2I benchmarks.

==> sections/related_work.tex <==
% \section{Related Work}
% \paragraph{Compositionality in Text-to-Image Generative Models}


% \paragraph{Compositional Generation with Large Language Models}
% \paragraph{Compositional Text-to-image Generation}
% Our work is also related to existing works that focus on 
% Most similar to our work, \cite{} propose to . In contrast, in our work, we aim to use 


%\paragraph{Compositional generative models}
% \cite{du2024compositionalgenerativemodelingsingle} argues that constructing complex generative models compositionally from simpler models can improve compositional performance.

% On the other hand, data augmentation~\citep{} and hard negative minings~\citep{} have been explored to improve text-image alignment in pre-trained VLMs. \paul{not sure these are the only 2 lines of previous work, seems like there are more. eg data augmentation, harder negatives, compositional generative modeling (see and cite yilun du's work)} 


% \cite{pandey2023crossmodalattentioncongruenceregularization} introduces Cross-modal Attention Congruence Regularization (CACR), a method designed to help models learn to align intra-modal relationships across different modalities more effectively.
% \cite{wang2024divideconquerlanguagemodels} introduces the use of an LLM as agent to guide image generation and reduce confusion among multiple objects. However, relying on external agents does not help the model develop an inherent understanding of compositionality.
